WizardMerge -- Save Us From Merging Without Any Clues

Modern software development necessitates efficient version-oriented collaboration among developers. While Git is the most popular version control system, it generates unsatisfactory version merging results due to textual-based workflow, leading to potentially unexpected results in the merged version of the project. Although numerous merging tools have been proposed for improving merge results, developers remain struggling to resolve the conflicts and fix incorrectly modified code without clues. We present WizardMerge, an auxiliary tool that leverages merging results from Git to retrieve code block dependency on text and LLVM-IR level and provide suggestions for developers to resolve errors introduced by textual merging. Through the evaluation, we subjected WizardMerge to testing on 227 conflicts within five large-scale projects. The outcomes demonstrate that WizardMerge diminishes conflict merging time costs, achieving a 23.85% reduction. Beyond addressing conflicts, WizardMerge provides merging suggestions for over 70% of the code blocks potentially affected by the conflicts. Notably, WizardMerge exhibits the capability to identify conflict-unrelated code blocks that require manual intervention yet are harmfully applied by Git during the merging.

==> Algorithms/GraphDebloating.tex <==
\begin{figure}[!t]
    \removelatexerror
    \begin{algorithm}[H]
        \caption{Graph Debloating (implemented as $graph\_debloating$)}
        \label{algorithm:graphdebloating}
            \algorithmicrequire Overall Dependency Graph $ODG$, current node $u$, previous preserved node $prev\_u$

            \algorithmicensure Shrinked Dependency Graph $SDG$
            
            $\vartriangleright make\_edge\left(a,b\right)$:\ return\ a\ new\ edge\ from\ $a$\ to\ $b$.
            
            $\vartriangleright visited\left(a, b\right)$:\ return\ whether\ node\ $a$\ with\ previously\ reached\ tagged\ node\ $b$\ has\ been\ visited.
            
            $\vartriangleright mark\_visited\left(a, b\right)$:\ mark\ node\ $a$\ with\ previously\ reached\ tagged\ node\ $b$\ has\ been\ visited.

            $\vartriangleright get\_end\_node\left(e\right)$:\ return\ the\ end\ node\ of\ edge\ $e$.

            $\vartriangleright is\_tagged\_with\_DCB\left(a\right)$:\ return\ whether\ node\ $a$\ has\ a\ DCB\ attached.

            \uIf{$visited\left(u, prev\_u\right) = false$ }
            {
                $mark\_visited\left(u, prev\_u\right)$
    
                \For{$e \in ODG$}
                {   
                    \uIf{$e\ starts\ from\ u$}
                    {
                        $v \xleftarrow{} get\_end\_node\left(e\right)$
                        
                        \uIf{$is\_tagged\_with\_DCB\left(u\right)$}
                        {
                            $SDG \xleftarrow{} make\_edge\left(prev\_u, u\right)$
                            
                            $graph\_debloating\left(ODG, v, u\right)$    
                       
                        }
                        \Else
                        {
                            $graph\_debloating\left(ODG, v, prev\_u\right)$  
                        }
                    }
                }
            }        
    \end{algorithm}
\end{figure}

==> Listings/error-applied-code.tex <==
% \begin{lstlisting}[label={lst:ex1}, language=C, caption={$x$, $y$, and $z$ represent three edges of a triangle, the vulnerable code will be executed when it is a right triangle.}]
% unsigned x, y, z = input();//input0: (x,y,z)=(1,2,3)
% if (x >= y && y >= z){//input1: (x,y,z)=(9,5,3)
%   if (y + z > x){//input2: (x,y,z)=(5,4,4)
%     if (y^2 + z^2 == x^2){//input3: (x,y,z)=(5,4,3)
%       // vulnerable code
%     } } }
% // other code
% \end{lstlisting}

\begin{figure}[t]
\captionsetup{type=lstlisting}
\caption{\textmd{An example of a clean but incorrect Git merge with the three-way merging algorithm.}}
\label{lst:vDCB_example}
\begin{lstlisting}[language=C]
int a = 1      /* [VA: // int a = 1;] | [VB: int a = 1;] */
int b = 2;
int c = 1 + b; /* [VA: int c = 1 + b;] | [VB: int c = a + b;] */
printf("%d", c);
\end{lstlisting}
\vspace{-0.6cm} 
\end{figure}


==> Sections/DataAvailability.tex <==
\section{Data Availability}

%
The source code of \sys and the evaluation datasets can be found at: \href{https://figshare.com/s/2f1269266a3aaab6c811}{https://figshare.com/s/2f1269266a3aaab6c811}.

==> Tables/Dataset_firefox.tex <==
\begin{table}
\label{tb:ffdataset}
\caption{\textmd{The final datasets information for evaluations on the research questions. \textbf{Conflicts Resolved Manually} indicates the number of conflicts resolved by Git merge only. \textbf{Conflicts Analyzed By \sys} indicates the number of conflicts resolved with the assistance of \sys. \textbf{Manually Merging Time Cost} and \textbf{Merge With \sys Time Cost} show the time consumption of merging these conflicts and the violated DCBs related to these conflicts w/ or w/o \sys respectively (accurate to minutes). }}

\begin{threeparttable}
\begin{tabular}{lllll}
\toprule
Dataset ID & MCR & ACR          & MCR TC & ACR TC          \\ \midrule
FF1        & 2                           & 2                                   & 3                          & 2                                  \\
FF2        & 2                           & 1                                   & 11                         & 6                                  \\
FF3        & 12                          & 12                                  & 49                         & 28                                 \\
FF4        & 11                          & 11                                  & 8                          & 5                                  \\
FF5        & 25                          & 25                                  & 32                         & 22                                 \\
FF6        & 26                          & 26                                  & 30                         & 27                                 \\
FF7        & 13                          & 13                                  & 42                         & 25                                 \\
FF8        & 3                           & 3                                   & 13                         & 8                                  \\
FF9        & 2                           & 2                                   & 2                          & 2                                  \\
FF10       & 9                           & 9                                   & 10                         & 10                                 \\
FF11       & 2                           & 2                                   & 4                          & 4                                  \\
FF12       & 3                           & 3                                   & 4                          & 3                                  \\
FF13       & 8                           & 8                                   & 16                         & 12                                 \\
FF14       & 1                           & 1                                   & 1                          & 1                                  \\
FF15       & 2                           & 2                                   & 2                          & 2                                  \\
FF16       & 1                           & 1                                   & 1                          & 1                                  \\
FF17       & 6                           & 6                                   & 6                          & 5                                  \\
FF18       & 12                          & 12                                  & 30                         & 19                                 \\
FF19       & 1                           & 1                                   & 1                          & 1                                  \\
FF20       & 3                           & 3                                   & 13                         & 8                                  \\
FF21       & 13                          & 13                                  & 59                         & 43                                 \\
FF22       & 3                           & 3                                   & 5                          & 4                                  \\ \bottomrule
\end{tabular}

\begin{tablenotes}
\footnotesize
\item[1] \sys-Async-CG1: \sys ablation control group one. The statistics are recorded with \sys running without multi-threaded constraint solving.
% \item[2] \sys-Async-CG2: \sys ablation control group two. The statistics are recorded with \sys running without state sharing between fuzzer and concolic executor backend.
\end{tablenotes}
\end{threeparttable}

\end{table}

==> Tables/Dataset_linux_kernel.tex <==
\begin{table}
\label{tb:lkdataset}
\caption{\textmd{The final datasets information for evaluations on the research questions. \textbf{Conflicts Resolved Manually} indicates the number of conflicts resolved by Git merge only. \textbf{Conflicts Analyzed By \sys} indicates the number of conflicts resolved with the assistance of \sys. \textbf{Manually Merging Time Cost} and \textbf{Merge With \sys Time Cost} show the time consumption of merging these conflicts and the violated DCBs related to these conflicts w/ or w/o \sys respectively (accurate to minutes). }}

\begin{threeparttable}
\begin{tabular}{lllll}
\toprule
Dataset ID & MCR & ACR          & MCR TC & ACR TC          \\ \midrule
LK1        & 1                           & 1                                   & 10                         & 5                                  \\
LK2        & 2                           & 2                                   & 31                         & 18                                 \\
LK3        & 5                           & 5                                   & 8                          & 5                                  \\
LK4        & 2                           & 2                                   & 5                          & 4                                  \\
LK5        & 5                           & 3                                   & 15                         & 10                                 \\
LK6        & 1                           & 1                                   & 3                          & 2                                  \\
LK7        & 2                           & 2                                   & 4                          & 4                                  \\
LK8        & 1                           & 1                                   & 2                          & 2                                  \\
LK9        & 1                           & 1                                   & 4                          & 4                                  \\
LK10       & 1                           & 1                                   & 2                          & 2                                  \\
LK11       & 4                           & 4                                   & 40                         & 33                                 \\
LK12       & 2                           & 2                                   & 6                          & 7                                  \\
LK13       & 1                           & 1                                   & 15                         & 8                                  \\
LK14       & 1                           & 1                                   & 8                          & 10                                 \\
LK15       & 1                           & 1                                   & 3                          & 3                                  \\
LK16       & 1                           & 1                                   & 1                          & 1                                  \\
LK17       & 1                           & 1                                   & 12                         & 11                                 \\
LK18       & 2                           & 2                                   & 2                          & 2                                  \\
LK19       & 2                           & 2                                   & 5                          & 10                                 \\
LK20       & 1                           & 1                                   & 1                          & 1                                  \\
LK21       & 1                           & 1                                   & 1                          & 1                                  \\
LK22       & 1                           & 1                                   & 1                          & 1                                  \\
LK23       & 2                           & 1                                   & 3                          & 2                                  \\
LK24       & 9                           & 6                                   & 30                         & 19                                 \\
LK25       & 5                           & 4                                   & 18                         & 13                                 \\
LK26       & 2                           & 2                                   & 3                          & 2                                  \\
LK27       & 1                           & 1                                   & 3                          & 3                                  \\
LK28       & 2                           & 2                                   & 2                          & 1                                  \\
LK29       & 1                           & 1                                   & 4                          & 3                                  \\
LK30       & 2                           & 2                                   & 8                          & 3                                  \\
LK31       & 1                           & 1                                   & 6                          & 4                                  \\
LK32       & 1                           & 1                                   & 1                          & 1                                  \\
LK33       & 1                           & 1                                   & 1                          & 1                                  \\
LK34       & 4                           & 4                                   & 10                         & 6                                  \\
LK35       & 1                           & 1                                   & 1                          & 1                                  \\
LK36       & 1                           & 1                                   & 2                          & 2                                  \\
LK37       & 1                           & 1                                   & 4                          & 4                                  \\
LK38       & 1                           & 1                                   & 1                          & 1                                  \\
LK39       & 1                           & 1                                   & 1                          & 1                                  \\
LK40       & 7                           & 7                                   & 10                         & 6                                  \\
LK41       & 1                           & 0                                   & 1                          & /                                  \\
LK42       & 2                           & 0                                   & 3                          & /                                  \\
LK43       & 3                           & 0                                   & 2                          & /                                  \\  \bottomrule
\end{tabular}

\begin{tablenotes}
\footnotesize
\item[1] \sys-Async-CG1: \sys ablation control group one. The statistics are recorded with \sys running without multi-threaded constraint solving.
% \item[2] \sys-Async-CG2: \sys ablation control group two. The statistics are recorded with \sys running without state sharing between fuzzer and concolic executor backend.
\end{tablenotes}
\end{threeparttable}

\end{table}

==> Tables/SOTA.tex <==
\begin{table}
\caption{\textmd{State-of-the-art merging systems list. }}
\label{tb:SOTASystems}
\begin{threeparttable}
\begin{tabular}{lll}
\toprule
\textbf{System Name} & \textbf{Type}    & \textbf{Language Supported}          \\ \midrule
JDIME                & Structured       & Java                                 \\
Mastery              & Structured       & Java                                 \\
Spork                & Structured       & Java                                 \\
SafeMerge            & Structured       & Java                                 \\
AutoMerge            & Structured       & Java                                 \\
FSTMerge             & Semi-Structured  & Scalable                             \\
IntelliMerge         & Semi-Structured  & Java                                 \\
SoManyConflicts      & Suggestion       & Java / JS\tnote{1} / TS\tnote{2}       \\
GMerge               & Machine Learning & C / C++                              \\ 
MergeBERT            & Machine Learning & C / C++                              \\ 
GMerge               & Machine Learning & C / C++                              \\ \bottomrule
\end{tabular}
\begin{tablenotes}
\footnotesize
\item[1] \textbf{JS}: JavaScript.
\item[2] \textbf{TS}: TypeScript.
\end{tablenotes}
\end{threeparttable}
\end{table}

==> Tables/vDCB_related_to_conflicts.tex <==
\definecolor{worse}{HTML}{FFCCC9}

\begin{table*}
\centering
\caption{\textmd{Conflict-related violated DCB records. \textbf{VA CR VDCB LoC} represents the number of lines of code of CR violated DCB in variant A, \textbf{VB CR VDCB LoC} represents the number of lines of code of CR violated DCB in variant B. The format of $n/m$ indicates that there are $m$ LoCs in total, of which \sys can detect $n$.}}
\label{tb:vDCB_related_to_conflict}

\resizebox{\textwidth}{!}{
\begin{tabular}{lllllllllllllllll}
\toprule
                     & \multicolumn{16}{c}{\textbf{Dataset ID}}                                                                                                                                                                                                                  \\ \cmidrule{2-17} 
                     & \textbf{FF5} & \textbf{FF6} & \textbf{FF7} & \textbf{FF8} & \textbf{FF10} & \textbf{FF13} & \textbf{FF14} & \textbf{FF15} & \textbf{FF16} & \textbf{FF17} & \textbf{FF18} & \textbf{FF20} & \textbf{FF21} &               &               &               \\ \midrule
\textbf{VA CR VDCB LoC} & 20/25        & 12/12        & 24/24        & 2/2          & 18/32         & 6/6           & 3/3           & 2/2           & 1/1           & 6/6           & 38/38         & 5/5           & 14/18         &               &               &               \\
\textbf{VB CR VDCB LoC} & 21/25        & 11/11        & 6/6          & 13/13        & 14/14         & 11/11         & 1/1           & 2/2           & 1/1           & 0/0           & 17/17         & 0/0           & 15/22         &               &               &               \\ \midrule
                     & \textbf{LK1} & \textbf{LK2} & \textbf{LK3} & \textbf{LK4} & \textbf{LK5}  & \textbf{LK7}  & \textbf{LK14} & \textbf{LK17} & \textbf{LK19} & \textbf{LK23} & \textbf{LK25} & \textbf{LK28} & \textbf{LK29} & \textbf{LK30} & \textbf{LK31} & \textbf{LK37} \\ \midrule
\textbf{VA CR VDCB LoC} & 4/4          & 10/13        & 4/4          & 0/2          & 47/47         & 2/2           & 4/4           & 10/10         & 1/1           & 8/8           & 0/19          & 8/8           & 1/1           & 3/3           & 4/4           & 1/1           \\
\textbf{VB CR VDCB LoC} & 2/2          & 8/11         & 5/18         & 0/1          & 0/0           & 3/3           & 22/22         & 1/1           & 2/2           & 9/9           & 0/19          & 1/1           & 1/1           & 3/3           & 91/91         & 8/8           \\ \bottomrule
\end{tabular}
}

\end{table*}

==> Tables/vDCB_unrelated_to_conflicts.tex <==
\definecolor{worse}{HTML}{FFCCC9}

\begin{table*}
\centering
\caption{\textmd{Conflict-unrelated violated DCB records. \textbf{VA CU VDCB LoC} represents the number of lines of code of CU violated DCB in variant A, \textbf{VB CU VDCB LoC} represents the number of lines of code of CU violated DCB in variant B. The format of $n/m$ indicates that \sys detect $m$ LoCs as CU violated DCB, of which $n$ are confirmed.}}
\label{tb:vDCB_unrelated_to_conflict}

\resizebox{\textwidth}{!}{
\begin{tabular}{llllllllllllll}
\toprule
                     & \multicolumn{13}{c}{\textbf{Dataset ID}}                                                                                                                                                                    \\ \cmidrule{2-14} 
                     & \textbf{FF5} & \textbf{FF7} & \textbf{FF10} & \textbf{FF11} & \textbf{FF12} & \textbf{FF18} & \textbf{FF20} & \textbf{FF21} & \textbf{}     & \textbf{}     & \textbf{}     & \textbf{}     & \textbf{}     \\ \midrule
\textbf{VA CU VDCB LoC} & 0/1          & 9/15         & 6/159         & 0/8           & 40/430        & 0/14          & 11/11         & 9/14          &               &               &               &               &               \\
\textbf{VB CU VDCB LoC} & 0/26         & 38/44        & 16/169        & 0/8           & 10/400        & 0/13          & 25/42         & 9/15          &               &               &               &               &               \\ \midrule
                     & \textbf{LK2} & \textbf{LK5} & \textbf{LK12} & \textbf{LK13} & \textbf{LK15} & \textbf{LK17} & \textbf{LK19} & \textbf{LK20} & \textbf{LK24} & \textbf{LK39} & \textbf{LK41} & \textbf{LK42} & \textbf{LK43} \\ \midrule
\textbf{VA CU VDCB LoC} & 10/10        & 40/224       & 23/23         & 2/2           & 52/788        & 1/1           & 8/14          & 4/49          & 0/8           & 0/6           & 1/1           & 5/92          & 25/27         \\
\textbf{VB CU VDCB LoC} & 9/9          & 0/108        & 0/0           & 2/2           & 48/683        & 1/1           & 3/9           & 5/61          & 0/6           & 0/18          & 1/1           & 14/97         & 22/25         \\ \bottomrule
\end{tabular}
}

\end{table*}
